Leveraging Unlabeled Data for Sketch-based Understanding

Sketch-based understanding is a critical component of human cognitive learning and is a primitive communication means between humans. This topic has recently attracted the interest of the computer vision community as sketching represents a powerful tool to express static objects and dynamic scenes. Unfortunately, despite its broad application domains, the current sketch-based models strongly rely on labels for supervised training, ignoring knowledge from unlabeled data, thus limiting the underlying generalization and the applicability. Therefore, we present a study about the use of unlabeled data to improve a sketch-based model. To this end, we evaluate variations of VAE and semi-supervised VAE, and present an extension of BYOL to deal with sketches. Our results show the superiority of sketch-BYOL, which outperforms other self-supervised approaches increasing the retrieval performance for known and unknown categories. Furthermore, we show how other tasks can benefit from our proposal.

==> images/conclusion.tex <==
\section{Conclusions}
In this work, we study how to handle unlabeled data to improve sketch retrieval. Our sketch-BYOL approach yields competitive results on known categories, and is the best performer for unknown categories. We also analyze our approach via embeddings visualizations, and sketch retrieval samples. Finally, we provide an application to retrieve (sketch, image) pairs for sketch-to-photo and sketch-based image retrieval tasks.

As future work, we plan to extend sketch-BYOL to manage sketch-based image retrieval via its two branches. The former one will encapsulate sketches, and the latter one will encapsulate images. Then, commonalities in these two modalities are extracted via the loss function.

% evaluate our approach in other NLP domains. Also, we will combine $Bert_{met+att}$ and $Fusion_{met+att}$ creating a new embedding combining course-guided attention, a embedding-guided attention ($Bert$, $Glove$, and $Word2vec$), and metric learning.
